Efficiently Quantifying and Mitigating Ripple Effects in Model Editing

Large Language Models have revolutionized numerous tasks with their remarkable efficacy. However, editing these models, crucial for rectifying outdated or erroneous information, often leads to a complex issue known as the ripple effect in the hidden space. While difficult to detect, this effect can significantly impede the efficacy of model editing tasks and deteriorate model performance. This paper addresses this scientific challenge by proposing a novel evaluation methodology, Graphical Impact Evaluation(GIE), which quantitatively evaluates the adaptations of the model and the subsequent impact of editing. Furthermore, we introduce the Selective Impact Revision(SIR), a model editing method designed to mitigate this ripple effect. Our comprehensive evaluations reveal that the ripple effect in the hidden space is a significant issue in all current model editing methods. However, our proposed methods, GIE and SIR, effectively identify and alleviate this issue, contributing to the advancement of LLM editing techniques.

==> latexs/00.CoverLetter.01.tex <==
% \section*{1. To All Reviewers}

% \subsection*{1.1 Clarity of GIE and SIR Explanations}

% We have reorganized the manuscript, with particular attention to the formulas in Sections 3 and 4. Given the complexity of GIE and SIR, a detailed summary is omitted here. In brief, we have reduced the use of symbols, making them more consistent, and started with the formula for Factual Change to explain how the evaluation methods for both Vanilla and GIE are conducted in the revised version.

% \subsection*{1.2 Conversion Between Triples and Prompts}

% To ensure consistency, we clarified in Section 3 that, during both the editing and evaluation processes, triples need to be converted into prompts. Specific examples are provided in the appendix. Since most model-editing approaches adopt a uniform method for converting triples into prompts, our focus lies on the selection of the triples themselves. Consequently, in subsequent formulas, we directly use the triple notation to represent the derived prompt, such as $f(\langle s, r, o \rangle)$, which stands for $f(\text{text}), \langle s, r, o \rangle \rightarrow \text{text}$.

% \section*{2. To Reviewer HuJZ}

% \subsection*{2.1 Source of the Vanilla Evaluation Method}

% We dedicated section* 4.1 to discussing the Vanilla Ripple Effect evaluation method and revisited its implementation in wiki30t in section* 5.1. In essence, the Vanilla method measures the change in perplexity of neighboring nodes in the knowledge graph before and after editing, while GIE constructs a network based on node similarity and compares the perplexity changes of neighboring nodes within this GIE network.

% \subsection*{2.2 Difficulty in Understanding Tables 1, 3, and 4}

% We have significantly condensed the content of Table~\ref{tab:simple_experiment}, moving all experimental results to the appendix in Table~\ref{tab:experiment}. Furthermore, for methods that do not modify model parameters (e.g., ICE, EREN, SERAC), their results have also been moved to the appendix since their principles differ from those of SIR and MEMIT, and thus, they are not directly comparable.

% The results from Table 1 can now be interpreted with focus on two key points:
% 1. Bold fonts highlight that GIE generally detects more significant Ripple Effects compared to Vanilla.
% 2. GIE's results tend to decrease as the number of hops increases, whereas the Vanilla method shows little correlation with hop count, indicating that GIE more accurately captures Ripple Effects.

% Tables 2 and 3 present the results of various model-editing methods applied to the GPT2-XL model:
% - Table 2 shows that SIR achieves higher editing accuracy compared to MEMIT and ICE.
% - Table 3 demonstrates that many methods cause the model to collapse after editing 50 facts, whereas SIR maintains good performance even after editing 200 facts.

% \section*{3. To Reviewer 1r2c}

% \subsection*{3.1 Comparison with Related Work and New Baselines}

% We have expanded our discussion of related works and included the results of EREN and SERAC in Table~\ref{tab:experiment}. However, due to significant differences between these methods and the model-editing approaches focused on in this paper, as well as the length of the table, these results are presented in the appendix. In brief, these methods rely heavily on the performance of a retriever model, which tends to become confused when editing large amounts of knowledge in a completely random setting, thereby affecting model outputs.

% As for the work of \citep{gangadhar2024model}, we were unable to replicate their experiments due to the lack of publicly available code. However, a detailed comparison is provided in the related works section*. Our research primarily focuses on analyzing the mechanism of Ripple Effect propagation through embedding-similar facts, attempting to mitigate its impact by breaking the propagation paths. In contrast, \citep{gangadhar2024model} primarily suppresses the Ripple Effect through objective function optimization.

% \subsection*{3.2 Common Evaluation Metrics}

% We used perplexity (PPL) as well as character-level metrics like BLEU and ROUGE, with detailed results presented in Figure 5 in the appendix. In the main text, we focus on PPL as it provides a more granular, probabilistic assessment, enabling a more precise evaluation of model performance.

% \subsection*{3.3 Evaluation Costs}

% In the revised version, we included a new figure, Figure~\ref{fig:sum_ppl_chng}, which illustrates the trade-off between Ripple Effect detection and evaluation costs. The results show that under dense knowledge editing (the first three green bars on the left side of each figure), SIR’s evaluation cost is only 5\% of that of Vanilla, while detecting 90\% of the total Ripple Effect. Further details are provided in the last paragraph of section* 6.1.

% \section*{4. To Reviewer de5n}

% \subsection*{4.1 Approximation Errors}

% We have added a new figure, Figure~\ref{fig:sum_ppl_chng}, depicting the differences in Ripple Effect detection across extensive experiments under different evaluation methods. 
% The results show that for weaker editing methods (e.g., FT), the perplexity change detected over the full knowledge graph (wiki5m) is approximately 1.25 times that of wiki30t. For stronger editing methods (e.g., MEMIT, SIR-Top5, and SIR-Top10), these methods reduce the Ripple Effect by enhancing model memory, thereby lowering global perplexity. For more details, see section* 6.1.

% \subsection*{4.2 Validity of Figure~\ref{fig.4}}

% We have revised the experimental analysis in section* 6.3:
% - Figure 4 analyzes the effect of SIR in mitigating Ripple Effect, based on the hypothesis that was verified in the experiments in Table 1. It shows changes in the Ripple Effect when SIR is applied to the top 5 or top 10 most relevant facts.
% - In both the left and right panels, lower perplexity indicates better performance.
% - The right panel shows that both methods effectively mitigate the Ripple Effect.
% - The left panel shows that applying SIR to the top 5 facts reduces global perplexity more than applying it to the top 10 facts. We hypothesize that the additional facts introduced in the top 10 scenario may reintroduce more Ripple Effects, causing perplexity to rise.

% \subsection*{4.3 Rationality of Object $o'$ in Triplet $\langle s, p, o \rangle$}

% The rationality of object $o$ in triplet $\langle s, p, o \rangle$ cannot always be guaranteed. Related works often deliberately introduce irrational $o$ values to test the performance of model-editing methods (e.g., \cite{cohen2024evaluating}, Version 1 injected the fact ``Eiffel Tower, city, London''). The goal of model-editing methods is to perform edits without altering other knowledge, regardless of the rationality of the target, which is a key evaluation criterion.

% In this paper, we adhere to this standard (see Step 3 in section* 5.1). The editing target maintains a certain degree of factual integrity. For instance, edits such as "Eiffel Tower is located in Trump" are not allowed. Each triplet $\langle s, r, o \rangle$ is modified to $\langle s, r, o' \rangle$, where $o'$ maintains the same relation $r$ as the original $o$.

\section*{1. To All Reviewers}

\subsection*{1.1 Clarity of GIE and SIR Explanations}

We have reorganized Section 3 and 4, particularly the formulas, to improve clarity.
The use of symbols has been minimized, and we now explain the evaluation methods for Vanilla and GIE seperately.

\subsection*{1.2 Conversion Between Triples and Prompts}

In Section 3, we clarified that triplets are converted into prompts for editing and evaluation, with examples provided in the appendix.
Since the focus of our method is on the triplet selection, so we directly use the triplet notation in formulas, such as $f(\langle s, r, o \rangle)$, which represents $f(\text{text}_{\langle s, r, o \rangle}).$  
% \rightarrow \text{text}$.

\section*{2. To Reviewer HuJZ}

\subsection*{2.1 Source of the Vanilla Evaluation Method}

Section 4.1 discusses the Vanilla Ripple Effect method, with implementation details in Section 5.1. Vanilla method measures the change in perplexity of neighboring nodes in the knowledge graph before and after editing. At the same time, GIE constructs a network based on node similarity and compares the perplexity changes of neighboring nodes within this GIE network.

\subsection*{2.2 Simplification of Tab.~\ref{tab:simple_experiment},~\ref{tab:case},~\ref{tab:case2}}

We condensed Table~\ref{tab:simple_experiment} and moved many experimental results to the appendix.
Especially methods that do not modify model parameters (e.g., ICE, EREN, SERAC).
Results show that GIE detects more significant Ripple Effects than Vanilla, with GIE's performance declining with increasing hops, while Vanilla shows no such correlation.
Tables 2 and 3 compare various editing methods on GPT2-XL, highlighting SIR's superior accuracy and stability even after editing 200 facts.

\section*{3. To Reviewer 1r2c}

\subsection*{3.1 Comparison with Related Work and Baselines}

We added results for EREN~\cite{chen2024robust} and SERAC~\cite{mitchell2022memory} in Tab.~\ref{tab:experiment} in appendix.
We do not find the code in \citet{gangadhar2024model}, so we only discuss the difference with their works in Secion 2.
Our work focused on how Ripple Effect happen and propagate, while theirs emphasize suppression through objective functions.

\subsection*{3.2 Evaluation Metrics}

Perplexity, BLEU, and ROUGE were used and displayed in Figure 5 (appendix).
Experiments in main content use PPL as the primary metric due to its probabilistic evaluation precision. 

\subsection*{3.3 Evaluation Costs}

We carried out a new experiment and displayed the result in Fig.~\ref{fig:sum_ppl_chng}.
Results show that SIR only evaluate on 5\% triplets of Vanilla's while detecting 90\% of Ripple Effects.
Detailed analysis is in Section 6.1.

\section*{4. To Reviewer de5n}

\subsection*{4.1 Approximation Errors}

We carried out a new experiment and displayed the result in Fig.~\ref{fig:sum_ppl_chng}.
Weaker methods detect higher global perplexity changes, while stronger methods like SIR reduce the Ripple Effect by enhancing model memory, thereby lowering global perplexity.

\subsection*{4.2 Validity of Figure~\ref{fig.4}}

Figure 4 illustrates that SIR reduces global perplexity more when applied to 5 relevant facts than to 10, as additional facts may reintroduce Ripple Effects.

\subsection*{4.3 Rationality of Object $o'$ in Triplet $\langle s, p, o \rangle$}

The rationality of object $o$ is not guaranteed, as irrational targets are sometimes used to test model-editing methods (e.g., \cite{cohen2024evaluating}). We adhere to the standard of maintaining factual integrity, modifying triples to $\langle s, r, o' \rangle$ where $o'$ holds the same relation as the original $o$.


\vspace{-3mm}
\bibliography{coverletter}

==> latexs/00Coverletter.tex <==
\section*{1. To All Reviewers}

\subsection*{1.1 GIE、SIR写得不够清楚}

我们重写了本文的表述，尤其是第三章和第四章的公式部分。
GIE和SIR部分的内容太多，这里就不做总结。
总而言之，我们在当前版本使用了更少，更规范的符号。并且来表示从Factual Change的公式~\ref{eq:factual_change}出发，Vanilla的评估方法和GIE的评估方法各自都是怎么进行的。

\subsection{1.2 Triplets and Prompt}

为了同一，我们在本文第三章节讲了编辑和评估都需要将三元组转换为Prompt，我们在Appendix给出了具体的例子。目前model editing对于三元组转换成prompt的方法都比较统一，而三元组的挑选才是本文的重点，所以之后的公式部分我们直接使用三元组符号来表示基于某个三元组改写来的prompt，如$f(\langle s,r,o\rangle)$表示的其实是$f(\text{text}), \langle s,r,o\rangle \rightarrow \text{text}$。


\section*{2. To Reviewer HuJZ}

\subsection*{2.1 Vanilla的评估方法是怎么来的}

我们在4.1章节单独开了一段来描述Vanilla Ripple Effect Evaluation Method。并在5.1章节重新表述了Vanilla评估方式是如何在wiki30t上进行的。
简而言之，Vanilla是直接去计算模型对于编辑目标在KG上的邻居在编辑前后的困惑度变化。
而GIE是基于KG中已有的节点，重新根据节点相似建了GIE Network，并在这个Network上对比编辑目标邻居在编辑前后的困惑度变化。

\subsection*{2.2 表1， 3， 4难以理解}

我们大幅删减了表~\ref{tab:simple_experiment}的内容，并将所有的实验结果放到了位于Appendix的表~\ref{tab:experiment}中。
除此之外，我们将所有不涉及模型参数修改的方法，如ICE、EREN、SERAC这些方法的实验结果也放到了Appendix中，因为这些方法和SIR、MEMIT等模型编辑方法的原理不同，可比性较低。

另外，我们重新表述了表1的实验结果，主要就是看表中表粗的部分，就是GIE能够检测出比Vanilla方法更强的Ripple Effect的地方。

Tables 2 and 3 present case studies, illustrating the output of various model editing methods after editing a given hard target in the GPT2-XL model.  
  - Table 2 shows that the well-known method, MEMIT, as well as the newer method, ICE, have a lower editing accuracy compare to SIR.
  - Table 3 demonstrates that many editing methods cause model collapse after editing 50 pieces of knowledge due to significant ripple effects. In contrast, the SIR method continues to perform well even after editing 200 pieces of knowledge.


\section*{3. To Reviewer 1r2c}

\subsection*{3.1 Comparsion with Related Work \& New baselines}

我们补充了相关工作，对于EREN~\cite{chen2024robust}和SERAC~\cite{mitchell2022memory}，我们将实验补充在了表~\ref{tab:experiment}中，但考虑到这两个方法，以及ICE和其他涉及参数修改的模型编辑方法存在较大差异，考虑到我们的main content中的表已经太过冗长，所以我们将这些实验移到了Appendix中。
简而言之，这两个通过将编辑目标存储到外部空间的方法，会非常依赖读取器模型的能力，尤其是在我们的Random设定下，即完全随机的要求200条知识编辑之后，读取器就会混乱，从而引发模型输出的混乱。

而对于\citep{gangadhar2024model}作而言，我们并没有找到这个工作的开源代码。
但依然在Related Work中进行了详细的比较。
我们的工作是希望发现怎样的编辑目标会影响到怎样的其他事实，并希望从Ripple Effect的影响路径上去切断这种影响。
而\citep{gangadhar2024model}工作主要是希望从目标函数上去抑制住这种Ripple Effect.

\subsection*{3.2 Common Evaluation Metrics}

We use perplexity alongside other character-level evaluation metrics such as BLEU and ROUGE.  
The detailed evaluation results can be found in Figure 5 in the appendix. We primarily use PPL in the main text because it provides more granular, probability-level results, which we believe offer more precise evaluations.


\subsection*{3.3 Evaluation Cost}

我们在这个版本绘制了一张新的图~\ref{fig:sum_ppl_chng}来展现各个评估方法之间所能检测到的ripple effect效果，以及所需要的开销。
结论是：如果编辑的知识比较密集（每张图的左边三个绿色柱子），SIR的评估开销可能只有Vanilla的5\%，却能精准地识别到Ripple Effect。
具体的实验介绍和分析可以参见6.1章节的最后一段内容。

\section*{4. To Reviewer de5n}

\subsection*{4.1 Approximation Error}


我们在这个版本绘制了一张新的图~\ref{fig:sum_ppl_chng}来展现在更大量的实验下，各个评估方法之间的ripple effect的差异。
结论是：对于较弱Model editing方法而言（如最左边的FT方法），全量KG上（wiki5m)所检测到的ppl变化大概是(wiki30t）的1.25倍。而对于较强的Model Editing方法而言（MEMIT、SIR-Top5, SIR-Top10)，这些方法为了降低ripple effect，往往会通过各种方法增强模型对已有知识的记忆，从而在全局上的ppl呈现降低的情况。
具体的实验介绍和分析可以参见6.1章节的最后一段内容。

\subsection*{4.2 Effectiveness in Fig.~\ref{fig.4}}

我们在6.3章节，对实验分析进行了重新表述：
- Figure 4 provides further analysis based on the premise that SIR effectively alleviate the Ripple Effect, a premise that is supported by the experiments shown in Table 1. Figure 4 analyzes how the Ripple Effect changes when SIR is applied to the 5 or 10 most relevant facts.  
- In both the left and right plots, a lower perplexity indicates better performance.  
- The right plot shows that both methods can effectively alleviate the Ripple Effect.  
- And the left plot shows that applying SIR to 5 facts leads to a greater reduction in global model perplexity than when applied to 10 facts. We speculate that the additional facts used in the 10-fact case may further introduce ripple effects, leading to the increase in perplexity.


\subsection*{4.3 Plausibility of o'}

The plausibility of ``o'' in the triple <s, p, o> cannot always be guaranteed.
In related work, it is often expected that ``o'' might not be plausible to create conflicts with existing facts and test model editing performance in extreme scenarios (for example, the v1 version of \cite{cohen2023evaluating} injected facts like ``Eiffel Tower, city, London'').  
The goal of model editing methods is to achieve the edit perfectly without altering other knowledge, regardless of the plausibility of the edit target itself, which is also important for model editing.  
In this paper, we adhere to the above standard (Step 3 in Section 5.1). Each target maintains a plausible degree of factual integrity (e.g., ``The Eiffel Tower is located in Donald Trump'' would not be a valid edit). For each triplet <s, r, o>, the edit target is modified to <s, r, o'>, where o' is chosen to maintain the same relation r as the original object o.



\bibliography{coverletter}

==> latexs/01Introduction.13.tex <==
% The swift advancement of Large Language Models~(LLMs) has exhibited remarkable efficacy across a multitude of tasks~\cite{brown2020language,zhao2023survey,openai2023gpt4,touvron2023llama,gu2023xiezhi}, yet the data embedded within these expansive models may become outdated or encompass errors~\cite{lazaridou2021mind,dhingra2022time, jang2022towards}.
% Methodologies for editing outdated and erroneous facts within LLMs have progressively garnered attention ~\cite{zhu2020modifying,de-cao-etal-2021-editing,meng2022locating,meng2023massediting,si2023prompting}.
% Model editing primarily aims to refine the factual memory of large language models (LLMs) in specific domains, ensuring improvements in targeted areas without compromising their overall factual accuracy.
% This process requires careful balancing to successfully implement factual edits while preventing unintended ripple effects damage the model's memorization towards other kinds of facts.


% Although many model editing techniques have proven effective in various situations, studies have shown that model editing deals damage to the LLMs' memory to other facts, which is called ``ripple effect''~\cite{gu2024model}. 
% The ripple effect is typically observed under circumstances where:
% First, knowledge editing introduces potential damage to the model's memory of other information about an entity after changing the model's understanding of that entity, known as the ``Ripple Effect in the Same Entity''~\cite{li2023unveiling,yao2023editing}.
% Additionally, changing the model's memory of an entity in a hidden space may also affect entities that are close in the hidden space, referred to as the ``Ripple Effect in Hidden Space''~\cite{hoelscherobermaier2023detecting,sakarvadia2023memory}.

% Ripple Effect in The Same Entity is relatively 直观 because there is actual factual connection between the entities within the edited facts and their candidate attributes or relations~\cite{cohen2023evaluating}.
% However, the Ripple Effect in Hidden Space, which lacks a direct factual connection with the edited object, presents a significant challenge in detection. 
% This implicit influence on other entities severely impedes the efficacy of all Model Editing method, culminating in a drastic deterioration in model performance as the quantity of edits escalates~\cite{li2023unveiling,wang2023knowledge}.

% 有效地量化评估不同model editing 方法所导致的ripple effect in hidden space是缓解该问题的第一步。
% In this study, we introduce a novel evaluative method, ed Graphical Impact Evaluation (GIE). 
% GIE facilitates a quantitative assessment of the Ripple Effects in Hidden Space engendered by model editing, thereby meticulously examining the adaptability of the model and the subsequent impacts of its modification.
% Specifically, GIE 从 Knowledge Graphs (KGs), which typically encapsulate a vast array of facts,中挑选编辑对象，并针对编辑对象的不同，针对性地挑选会被最大影响的其他事实性知识进行评估。
% This design come from one of our findings, which indicate that model editing preferentially impacts other facts that possess embeddings similar to the edited facts.
% 通过评估模型对于这些最容易受到影响的事实的变化，GIE可以量化地评估Ripple Effect in Hidden Space.

% Building upon the concept of GIE, we further propose an efficient and effective method to mitigate the ripple effects, named Selective Impact Revision (SIR).
% SIR suppresses the ripple effects of model editing by selecting and retraining facts in the KG that is closely related to the edited facts during the model editing process.

% GIE discovered that even the state-of-the-art (SOTA) model editing method still suffer from severe ripple effect in the hidden space with 16.51\% unrelated facts severely affected.
% SIR mitigates such issues by reducing the performance decrease of the SOTA model editing method in the ripple effect in the hidden space by 54.75\%.


The rapid progress of Large Language Models (LLMs) has demonstrated remarkable effectiveness across a wide range of tasks~\cite{brown2020language,zhao2023survey,openai2023gpt4,touvron2023llama,gu2023xiezhi}. 
However, the vast amount of facts embedded within these models may become outdated or contain errors~\cite{lazaridou2021mind,dhingra2022time, jang2022towards}.
As a result, methods for editing these facts within LLMs have gained increasing attention~\cite{zhu2020modifying,de-cao-etal-2021-editing,meng2022locating,meng2023massediting,si2023prompting}.
The primary goal of model editing is to refine the factual memory of LLMs in specific domains, ensuring targeted improvements without compromising overall factual memorization accuracy.
This process requires a delicate balance to successfully implement factual edits while preventing unintended damage to the model's memorization of other facts.

Despite the effectiveness of many model editing techniques in various situations, studies have revealed that model editing harms the LLMs' memory of other facts, a phenomenon known as the ``ripple effect''~\cite{gu2024model}.
The ripple effect manifests in two primary forms:
``Ripple Effect in the Same Entity'' and ``Ripple Effect in Hidden Space''.
The former occurs when editing knowledge about an entity potentially damages the model's memory of other facts related to that entity~\cite{li2023unveiling,yao2023editing}.
The latter arises when changing the model's memory of an entity in a hidden space affects other entities close to it in that space~\cite{hoelscherobermaier2023detecting,sakarvadia2023memory}.


The Ripple Effect in Hidden Space plays a crucial role in the efficacy of model editing techniques, as it lead to a cascade of unintended consequences that severely undermine the performance of the edited models~\cite{li2023unveiling,wang2023knowledge}. 
However, unlike the Ripple Effect in the Same Entity, which is relatively straightforward to detect due to the explicit factual connection between the edited facts and their candidate attributes or relations~\cite{cohen2023evaluating}, the Ripple Effect in Hidden Space presents a significant challenge in detection.
The absence of a direct factual link with the edited object makes it difficult to identify and mitigate the implicit influence on seemingly unrelated entities.
As the number of edits grows, failing to address the Ripple Effect in Hidden Space results in a drastic decline in model performance, rendering the edited models unreliable and potentially harmful when deployed in real-world applications.
Therefore, detecting and mitigating the Ripple Effect in Hidden Space is paramount for ensuring the reliability and practicality of model editing techniques.



To address this challenge, we first introduce a novel quantitative evaluation method called Graphical Impact Evaluation (GIE). 
Specifically, GIE selects edit targets from Knowledge Graphs (KGs), which typically contain many facts, and evaluates the most significantly affected factual knowledge based on the differences in edit targets. This design stems from one of our findings, which indicates that model editing preferentially impacts other facts with embeddings similar to the edited facts.
By evaluating the model's changes in response to these most easily influenced facts, GIE effectively and efficiently assess the Ripple Effect in Hidden Space.

Building upon the concept of GIE, we further propose an efficient and effective method to mitigate the ripple effects, named Selective Impact Revision (SIR). 
SIR suppresses the ripple effects of model editing by selecting and retraining facts in the KG that are closely related to the edited facts during the model editing process.
By focusing on the most relevant facts identified through GIE, SIR efficiently targets the root cause of the ripple effect and effectively minimizes its impact on the model's performance.

The GIE method revealed that even the state-of-the-art (SOTA) model editing approach is significantly impacted by ripple effects in the latent space, with 16.51\% of unrelated facts experiencing severe consequences.
The SIR method demonstrated a 54.75\% reduction in the intensity of the ripple effect within the hidden space compared to the SOTA model editing technique.

%SIR mitigates such issues by reducing the performance decrease of the SOTA model editing method in the ripple effect in the hidden space by 54.75\%.


% GIE enables a quantitative assessment of the Ripple Effects in Hidden Space caused by model editing, allowing for a thorough evaluation of the roby and the consequences of its modification.


% The Ripple Effect in the Same Entity is relatively straightforward to detect due to the explicit factual connection between the edited facts and their candidate attributes or relations~\cite{cohen2023evaluating}.
% In contrast, the Ripple Effect in Hidden Space presents a significant challenge in detection because there is no direct factual link with the edited object.
% This implicit influence on seemingly unrelated entities leads to a cascade of unintended consequences, severely undermining the effectiveness of all model editing methods and resulting in a drastic decline in model performance as the number of edits grows~\cite{li2023unveiling,wang2023knowledge}.
% Detecting and mitigating the Ripple Effect in Hidden Space is crucial for ensuring the reliability and practicality of model editing techniques. Failing to address this issue renders the edited models unreliable and potentially harmful when deployed in real-world applications.


% In summary, this paper has made the following contributions:
% \begin{itemize}
% \item We pioneer the exploration of the Ripple Effect in Hidden Space, a detrimental yet implicit phenomenon in model editing, and emphasize its critical importance in ensuring the reliability and practicality of edited models in real-world applications.
% \item We introduce GIE, a specialized technique for quantitatively evaluating the Ripple Effect in Hidden Space during model editing, effectively detecting this effect across various model editing methods.
% \item Leveraging the fundamental design of GIE, we develop SIR, an innovative model editing method that employs existing knowledge graphs to mitigate the Ripple Effect in Hidden Space, consistently outperforming other model editing methods in our experiments.
% \item We conduct comprehensive evaluations and comparative experiments, demonstrating the effectiveness of GIE in identifying the Ripple Effect in Hidden Space and the superior performance of SIR in alleviating this issue compared to other model editing techniques.
% \end{itemize}

==> latexs/03Preliminary.6.tex <==
\textbf{Knowledge Graph (KG}) is a large-scale semantic network that includes all kinds of factual knowledge.
It consists of entities and the various semantic relationships between them.
KGs use collections of triplets to describe entities and their relationships.
A triplet $\langle s, r, o\rangle$, the fundamental unit of knowledge representation in a KG, typically consists of a subject, relation, and object, representing either the relationship between entities or an attribute value of an entity.

\textbf{Model Editing} is a method that focuses on applying factual updates to language models (LMs). This approach involves converting an edit target, represented as a triple $\langle s_e, r_e, o_e\rangle$, into a free-text prompt. The existing LM, denoted as $f_\theta$, is then fine-tuned using this prompt to incorporate the new factual information while maintaining its pre-existing knowledge and capabilities~\cite{cohen2023evaluating}.

\textbf{Factual Change} refers to the overall changing of the LM's memorization of factual knowledge.
Given a fact set $\mathcal{F}$ and a corresponding set of changes $\Delta \mathcal{F} (|\Delta \mathcal{F}| \leq |\mathcal{F}|)$, the post-change fact set in LM is expressed as
\vspace{-3mm}
\begin{equation}
   \mathcal{F'} = \mathcal{F} + \Delta \mathcal{F} + R(\Delta \mathcal{F}),
\vspace{-3mm}
\end{equation}
where $R(\Delta \mathcal{F})$ signifies the ripple effect induced by $\Delta \mathcal{F}\vspace{2mm}$.

% \gzh{find a right position to stress that $R(\Delta F)$ is mostly harmful to the model.}

\textbf{Ripple Effect}, a side effect of model editing, arises from modifications to a language model's memory of specific factual knowledge, causing changes in the model's internal parameters and consequently impacting its memory of other factual knowledge. Specifically, the Ripple Effect can be divided into two types: the Ripple Effect in the Same Entity ($R_E$) and the Ripple Effect in Hidden Space ($R_H$). The overall impact of the Ripple Effect can be represented as $R=R_E+R_H$.

% 这是模型编辑所带来的副作用。
% 起因是改变语言模型对于某个事实知识的记忆，会导致模型内部的参数发生变动，从而影响到对于其他事实知识的记忆。
% 具体而言，Ripple Effect可以分为两个类型：
% Ripple Effect in The Same Entity $R_E$和 Ripple Effect in Hidden Space $R_H$。
% 而整体的Ripple Effect的效果可以表示为$R=R_E+R_H$。

% an observable phenomenon within KGs, is characterized by the spread of a single fact alteration throughout the interconnected node network, leading to subsequent changes in various nodes and underlining the interconnected nature of factual information.
% This phenomenon exhibits a more intricate nature in LLMs, where it can be delineated into two distinct categories. 
% Each category represents a unique pathway of influence in the model's response to factual changes, demonstrating how modifications in one part of the network can affect the whole system in varied ways. The aggregate ripple effect $R$ is computed as: $ R = R_E + R_H $, capturing the comprehensive impact of fact changes across different dimensions.

\textbf{Ripple Effect in The Same Entity $R_E$}: 
This is the phenomenon where modifications to the facts of an entity result in changes to other facts related to the same entity.
Ideally, factual updates made within a model should not impact unrelated parts of the same entity.
However, current prevalent model editing techniques often display a high sensitivity to changes within entities, inadvertently causing collateral modifications. 
% This tendency for interdependent changes characterizes the $R_E$ phenomenon.

\textbf{Ripple Effect in Hidden Space $R_H$}: 
This phenomenon describes a scenario where changes to a specific fact provoke unexpected alterations in seemingly unconnected facts and entities.
This effect is attributed to the proximity of different entities and facts within the latent embedding space. 
Therefore, updates to parameters in one area unintentionally harm the model's performance regarding other facts due to these underlying interconnections within the embedding space.







==> latexs/04OurMethod.7.tex <==
% Our methodology unfolds in two sub-sections, each tailored to systematically advance the accuracy and relevance of the model's knowledge base.

\subsection{Graphical Impact Evaluation~(GIE)}

To evaluate the ripple effect caused by model editing, an evaluation metric is first required to calculate the model's confidence score for a given fact.
In the main paper, we used {perplexity (ppl)~\cite{jelinek1977perplexity} as the evaluation metric, while {BLEU~\cite{papineni2002bleu} and ROUGE~\cite{lin2004rouge} are employed in the Appendix~\ref{sec:appendix2}.
The ripple effect $E$ introduced by model editing can be quantified by measuring the change in the evaluation metric on all fact memory that is not the edited target within the edited LLM, computed by the post-edit model \(f_{\theta_e}\) and the pre-edit model \(f_\theta\):
% \vspace{-2mm}
\begin{equation}
    E = \text{Metric}[f_{\theta_e}(\mathcal{F'}\setminus\Delta \mathcal{F})] - \text{Metric}[f_\theta(\mathcal{F})].
    \label{eq:ripple_effect_on_facts}
% \vspace{-2mm}
\end{equation}

However, obtaining all factual knowledge is extremely challenging. 
Directly using existing KGs to evaluate the Ripple Effect quantitatively is an alternative.
Existing KGs contain vast factual knowledge and have undergone manual or automated validation to ensure quality. 
It also provides a standardized testing benchmark for evaluating various model editing methods.
For a fact triplet that are not the edited target $ \langle s, r, o\rangle \notin \Delta \mathcal{F} $ in the KG, equation~\ref{eq:ripple_effect_on_facts} is rewritten by GIE as:
% \vspace{-2mm}
\begin{equation}
    E = \text{Metric}[f_{\theta_e}(\langle s, r, o\rangle )] - \text{Metric}[f_\theta(\langle s, r, o\rangle )]
% \vspace{-2mm}
\end{equation}
where $\langle s, r, o\rangle$ is the input prompt describing $s$, $r$ and $o$.

However, directly using the entire KG is precise yet highly inefficient.
GIE proposes to assess the metric changing in the triplets most similar to the edit targets to efficiently evaluate the ripple effect.
This method is premised on the observation that knowledge most related to the edit targets exhibits the greatest variance in model editing.
By quantifying the degree of change in these closely related triplets, the impact of the model editing can be effectively yet efficiently assessed, thereby measuring the Ripple Effect:
% \vspace{-2mm}
\begin{equation}
\small
S_{\text{selected}} = \text{sim}\left(f_{\theta}\left(\langle s_e, r_e, o_e \rangle\right), f_{\theta}\left(\langle s, r, o \rangle\right)\right) > \tau ,
\end{equation}
% \begin{equation}
%     \langle s_e, r_e, o_e \rangle \in \mathcal{KG}\cap\Delta\mathcal{F} \mid \langle s, r, o \rangle \in \mathcal{KG}\setminus \Delta\mathcal{F}
% \end{equation}
% \vspace{-5mm}
% \footnotesize{
\begin{align}
E& = \frac{1}{|S_{\text{selected}}|}
  \sum_{\langle s, r, o \rangle \in S_{\text{selected}}} \notag\\
  &\left( \text{Metric}[f_{\theta_e}(\langle s, r, o \rangle)] - \text{Metric}[f_\theta(\langle s, r, o \rangle)] \right)
\end{align}
% }
% where $f_\theta(\langle s, r \rangle)$ denotes the embedding vector of the triplet $\langle s, r \rangle$ under the pre-edit model $f_{\theta}$.
where $\langle s_e, r_e, o_e \rangle$ denotes the triplets of edit targets.
$\text{sim}(\cdot,\cdot)$ is an embedding similarity function, and $\tau$ is a threshold defining the minimal similarity for inclusion in the evaluation set $S_{\text{selected}}$.



% 然而，直接使用整个KG去做评估虽然测的准，但效率也太大了。
% GIE提出可以可以直接利用三元组在被编辑的模型中的向量相似度来挑选embedding最相似的三元组进行评估：
% <公式>
% 这是因为我们发现，当模型被编辑的时候，和编辑知识最相关的其他知识受到的影响最大。
% 通过测量这些知识的变化程度，可以有效判断模型编辑方法对于其他知识的影响程度，进而测量Ripple Effect.



\subsection{Selective Impact Revision~(SIR)}


The simplest method to mitigate the Ripple Effect is to retrain the model using all facts memorized by LMs except the edit target. 
% \vspace{-2mm}
\begin{equation}
\min_{\theta} \sum_{f \in \mathcal{F'} \setminus \Delta\mathcal{F}} \mathcal{L}(f; \theta)
% \vspace{-2mm}
\end{equation}
where \( \mathcal{L} \) is the loss function and \( \theta \) represents the model parameters. This approach aims to preserve the memory of all other facts while accommodating the edited facts.

However, as discussed in the GIE subsection, obtaining the memory of an LLM for all facts is extremely challenging.
Therefore, directly using existing comprehensive KGs as a surrogate  of all facts is a practical compromise:
% \vspace{-2mm}
\begin{equation}
\min_{\theta} \sum_{\left ( s,r,o\right ) \notin \Delta\mathcal{F}} \mathcal{L}(\langle s,r,o \rangle; \theta)
\end{equation}
Nevertheless, existing KGs often consist of billions of triplets of facts.
Retraining the entire model on all facts from the KGs every time a model edit is performed incurs significant computational overhead.

SIR proposes a more efficient approach by selectively retraining based on the degree of confidence score change between the edited and pre-edited LLMs regarding the facts in the KGs.
For an edited model \( f_{\theta_e} \), the fact triplets that suffer the most from the ripple effect are detected by the GIE method. Let \( \delta = \text{Metric}[f_{\theta_e}(\langle s,r,o\rangle)] - \text{Metric}[f_\theta(\langle s,r,o\rangle)] \) represent the change in the evaluation metric for triplet \( \left( s, r, o \right) \) before and after editing. 
SIR samples the top-K facts with the largest \( \delta_i \) values and re-edits these facts.
So, the SIR training objective can be formulated as follows:
% \vspace{-3mm}
\begin{equation}
\min_{\theta} \sum_{f \in \mathcal{O}} \mathcal{L}(f; \theta)
\end{equation}
where \( \mathcal{O} \) is the set of top-K facts with the largest \( \delta_i \) values:
\begin{equation}
\small{
\mathcal{O} = \{ \langle s,r,o\rangle \mid \delta \text{ is among the top-K largest changes} \}.}
\end{equation}

% As the number of edit requests increases, the performance of model editing methods typically decreases. However, SIR ensures that the model retains the most vulnerable knowledge, thereby improving accuracy across all facts.

% \blue{WJC: I changed some equations, using $\langle s, r\rangle$ for prompts, \( \left( s, r, o \right) \) for triplet, please check if there are any problems.}



% \begin{wrapfigure}{R}{0.5\textwidth}
% \vspace{-20pt}
% \centering
% % \includegraphics[width=\linewidth]{fig/figure1.png} 
% \includegraphics[width=\linewidth]{fig/metric_distribution.png}

% \caption{
% The frequency distribution of perplexity differences
% }
% \label{fig:metric_dis}
% \vspace{-35pt}
% \end{wrapfigure}

% Figure~\ref{fig:metric_dis} shows the frequency distribution of perplexity changes before and after typical model edits.
% The figure indicates that the changes in the evaluation metric roughly follow a normal distribution.
% Thus, an outlier knowledge triplet can be defined as a triplet whose evaluation metric change exceeds a certain threshold, specifically: $ \delta > \mu + 2\sigma $.
% Here, $\delta$ represents the change in the evaluation metric before and after editing, $\mu$ is the mean, and $\sigma$ signifies the standard deviation.



==> latexs/06Experiment.3.tex <==


\input{tables/error_approximation_table}

\subsection{Overall Ripple Effects Evaluation}

\textbf{Ripple Effect Differs on Both Different Edit Quantities and Distributions.}  
As shown in Tab.~\ref{tab:simple_experiment}, the evaluation results indicate that model performance is influenced by both the quantity and the distribution of the edits. The intensity of the ripple effect escalates with an increasing number of edits; under identical edit quantities, the ripple effect is generally more pronounced in breadth-first search (BFS) distributed edits than randomly distributed edits.

\textbf{Excessive Edits Lead to Model Deterioration.}  
The performance of ROME and MEND significantly deteriorates when the number of edits exceeds 50. Although FT+L appears stable in Tab.~\ref{tab:simple_experiment}, it is not a practical approach as its updating mechanism restricts weight adjustments, thereby hindering the efficient update of parameters and the generation of meaningful sentences, as evidenced in Tab.~\ref{tab:case2}.

\textbf{GIE Detects Heavier Ripple Effects on Most Baselines than Vanilla.}
From Tab.\ref{tab:simple_experiment}, it is evident that proximity within the original KG used by Vanilla does not always result in a more significant ripple effect when compared to the similarity graph used by GIE.
This challenges the assumption that ``closer nodes are necessarily more affected by editing''~\cite{cohen2023evaluating}.
We draw a conclusion that there is no consistent correlation between distance on the original KG and reduced model performance.
Both nearby and distant triplets experience substantial ppl changes following model edits.

The GIE method, which evaluates ripple effects using the similarity graph, is designed to minimize the semantic distance between triplets affected by the edits, while increasing the distance between unaffected triplets and the edited ones.
As demonstrated by the bolded values in Tab.~\ref{tab:simple_experiment}, triplets closer to the edit target in the similarity graph exhibit greater increases in perplexity compared to the original KG evaluated by Vanilla, whereas nodes with no direct connections show a smaller increase in perplexity.
This demonstrates the higher sensitivity of GIE in detecting ripple effects.

The underlined values in Tab.~\ref{tab:simple_experiment} highlight the differences in perplexity changes between GIE, which uses the similarity graph, and Vanilla, which uses the original KG. 
For example, in the BFS method under a single edit, the distinction between the similarity graph in GIE and the original KG in Vanilla is particularly notable, showing that GIE captures the ripple effects more effectively by considering the semantic relationships between triplets.
In contrast, the ripple effects observed in Vanilla, which relies on direct connections in the original KG, are often less pronounced or even negative, as seen in subsequent entries of the same row.

% \textbf{GIE Detect Heavier Ripple Effect on Most Baselines than Vanilla.}  
% Moreover, the experiment examines the impact of similarity between edited and pre-edit triplets. From Tab.~\ref{tab:experiment}, it can be deduced that proximity on the vanilla KG does not always result in a more significant ripple effect compared to the GIE network, challenging the inherent assumption that “closer nodes are necessarily more affected by editing”~\cite{cohen2023evaluating}. There is no consistent correlation between distance on the vanilla KG and decreased performance. Both proximate and distant triplets are susceptible to changes following model editing.

% The objective of the GIE network is to minimize the distance between triplets affected by the “ripple effect in hidden space” and the edited triplets while simultaneously increasing the distance between unaffected triplets and the edited ones. As the bolded numbers in Tab.~\ref{tab:experiment} demonstrate, triplets in closer proximity to edit targets in the GIE network exhibited an increase in perplexity, while nodes with no connectivity showed a decrease in perplexity relative to the vanilla KG, highlighting the effectiveness of our proposed GIE method.

% The underlined numbers in Tab.~\ref{tab:experiment} specifically highlight the differential change in perplexity under the GIE method compared to the vanilla KG. For instance, in the BFS method under 1 edit, the difference between the vanilla KG and GIE underscores a significant discrepancy when the hidden aspects of data are considered. It indicates that the influence of the ripple effect in hidden space is markedly more significant than in the same entity, where the difference was either less pronounced or negative, as observed in the subsequent entries of the same row.



\subsection{In-depth Comparison towards Two Types of Ripple Effect}


The vanilla KG is instrumental in measuring the ripple effect within the same entity.
Conversely, the GIE Network effectively captures ripple effects within latent spaces.
By reconstructing the overall ripple effect into another network, we can assess the relative contribution of each type of ripple effect to the overall deterioration of model performance.

To investigate this, we employ MEMIT, the state-of-the-art model editing method, to construct a Ripple Network.
This network is built through an iterative process that involves editing facts, identifying the most affected entities, and establishing connections between these entities and the edited ones.
The process is repeated 100 times to ensure comparable scale and structure between the Ripple Network of MEMIT and the vanilla KG.

Despite having similar edge counts (\(10^4\)) and densities, the two graphs exhibit significant structural divergence. To quantify this dissimilarity, we utilize Graph Edit Distance (GED), a metric that assesses the impact of alterations on the structural integrity and informational consistency of knowledge graphs. We calculate a simplified version of GED using the L1-norm:
% \vspace{-2mm}
\[
\text{GED} = \log\left( \left| \mathbf{G}_{\text{adj}} - \mathbf{G'}_{\text{adj}} \right| \right),
% \vspace{-2mm}
\]
where \(\mathbf{G}{\text{adj}}\) and \(\mathbf{G'}{\text{adj}}\) represent the adjacency matrices of the two graphs, respectively.

Fig.~\ref{fig.2} illustrates the evolution of GED across iterations for different network configurations. 
The initial high GED is attributed to the absence of links in the Ripple Network of MEMIT at iteration 0.
As the iterations progress, the GED between Ripple Network and GIE Network gradually decreases, indicating that the GIE Network's structure becomes increasingly similar to that of the Ripple Network. 
It suggests that the Ripple Effect in Hidden Space significantly contributes to the overall decrease in model performance.
Conversely, the GED between the Ripple Network and the vanilla KG continues to increase, implying that the vanilla KG contains numerous unrelated links and is not well-suited for detecting the ripple effect.

Fig.~\ref{fig.3} presents the frequency distribution of node degrees for the three networks. 
The vanilla KG exhibits a rapidly declining frequency of higher node degrees, a characteristic common in real-world networks. 
In contrast, the Ripple Network of MEMIT displays a more uniform distribution across various node degrees, indicating a more evenly distributed connectivity. 
Interestingly, the structure of the GIE Network more closely resembles that of the vanilla KG rather than the Ripple Network, suggesting potential for further improvement in the GIE method.

% The vanilla Knowledge Graph (KG) is instrumental in measuring the ripple effect within the same entity. Conversely, the Graph Inductive Embedding (GIE) Network effectively captures ripple effects within latent spaces. By reconstructing these impacts into distinct graphs, we can quantify the contribution of each type of ripple effect to the overall decline in model efficacy through structural differences.
% By reconstructing the impacts induced by the Ripple Effect into a new graph and measuring the structural differences between these graphs, it is possible to ascertain the extent to which each type of Ripple Effect contributes to the overall degradation of model performance in model editing.

% The MEMIT, which is the SOTA model editing method in previous researches, is employed to construct the Ripple Network, hereafter referred to as the Ripple Network of MEMIT.
% This network is developed through an iterative process involving editing facts, identifying the most affected entities, and establishing links between these entities and the edited entities.
% This process is repeated 100 times to ensure consistency in scale and structural comparisons between the Ripple Network of MEMIT and the vanilla KG.
% Although both graphs contain approximately \(10^4\) edges and exhibit similar densities, their structural details significantly diverge.


% Graph Edit Distance (GED) is utilized as a metric to determine the similarity between two graphs, providing insights into how alterations affect the structural integrity and informational consistency of knowledge graphs. 
% We calculate a simplified version of GED using the L1-norm:
% \[
% \text{GED} = \log\left( \left| \mathbf{G}_{\text{adj}} - \mathbf{G'}_{\text{adj}} \right| \right),
% \]
% where \(\mathbf{G}_{\text{adj}}\) and \(\mathbf{G'}_{\text{adj}}\) denote the adjacency matrices of two graph, respectively.




% Fig.~\ref{fig.2} illustrates the change in GED across iterations between different network configurations.
% Since there has no links in the 0 iteration of Ripple Network of MEMIT, so the GED in starting point is high.
% Then GED between the GIE Network and the Ripple Network of MEMIT gradually declines, suggesting that the GIE Network has closer structure to the Ripple Network, suggest that Ripple Effect in Hidden Space contribute a lot in overall model performance decreasing.
% While the GED between GIE Network and the Vanilla KG keep on increasing, suggesting that vanilla KG contain too many unrelated link, it is poor to use vanilla KG to detect the Ripple Effect.


% Fig.~\ref{fig.3} depicts the frequency distribution of node degrees for three networks.
% The vanilla KG shows a rapidly declining frequency of higher node degrees, typical of real-world networks.
% he Ripple Network of MEMIT displays a more uniform distribution across a range of node degrees, suggesting a more evenly distributed connectivity.
% The Structure of GIE Network is more similar to Vanilla KG but not Ripple Network, suggesting that GIE method still has room for further improvement.


% In contrast, t exhibits pronounced peaks at specific node degrees, indicating targeted alterations in node connectivity due to the ripple effect.



% The experimental results elucidate the distinct behaviors and impacts of ripple effects in KGs. The Ripple Network of MEMIT significantly aligns its structure closer to the vanilla KG over iterations, demonstrating the effectiveness of MEMIT in mitigating the initial discrepancies. On the other hand, the GIE Network consistently maintains a structural similarity with the vanilla KG, suggesting its robustness in preserving information consistency despite modifications. Collectively, these findings highlight the differential impacts of ripple effects and the potential of specific methodologies like MEMIT in managing these dynamics within KGs.


% vanilla KG可以有效测量Ripple Effect in The Same Entity.
% GIE Network可以有效测量Ripple Effect in Hidden Space.
% 将Ripple Effect所带来的影响再建成一张图，那么通过衡量这些图的结构差异，就可以发现这两种Ripple Effect对于Model Editing所带来的模型能力总体下降的贡献度。


% The difference is calculated by Graph Edit Distance~(GED) serves as a metric to gauge the similarity between two graphs, offering insights into how modifications affect the structural integrity and informational consistency of knowledge graphs.
% We compute a simplified version of GED between the GIE network and the vanilla KG using $\mathcal{L}{\textit{1}}-\textit{\text{norm}}$:
% \vspace{-2mm}
% \begin{equation}
% \centering
% \text{GED} = \log\left( \left| \mathbf{G}{\text{adj}} - \mathbf{G'}{\text{adj}} \right|\right),
% \end{equation}
% where $\mathbf{G}{\text{adj}}$ and $\mathbf{G'}{\text{adj}}$ denote the adjacency matrices of the vanilla KG and GIE network, respectively.

% 我们使用编辑效果最好的MEMIT来将Ripple Effect构建成Network，为了方便称呼，便称其为Ripple Network of MEMIT.
% The iterative process to build the Ripple Network of MEMIT involves editing facts, identifying the nodes that most effected by the editing, and establishing connections between these outliers and the edited triplets. This process is repeated 100 times to ensure consistency in the scale and structure comparisons between the Ripple Network of MEMIT and the vanilla KG. 
% Despite both graphs having approximately $10^4$ edges and similar density, their structural details diverge significantly.

% The GED As illustrated in Fig.~\ref{fig.2}, 

% The degree distributions of both graphs is differed as shown in Fig.~\ref{fig.3}.
% The vanilla KG displays a skew towards lower degrees, indicating a denser core, whereas the GIE network exhibits a more uniform degree distribution.
% This observation underscores the impact of edits on the structural diversity of the graph, suggesting that the GIE network may be better equipped to handle diverse informational contexts without a central density bias.

% These findings lead to a profound conclusion that, while the GIE network structurally diverges from the vanilla KG as evidenced by increasing GED values over iterations, it potentially offers a superior representation.
% This enhanced representation capability highlights the ``ripple effect in hidden space'' more effectively than the vanilla KG, challenging the notion that proximity in the traditional knowledge graph structure correlates directly with model performance~\cite{zhang2019graph}.
% Instead, the adaptability and structural evolution of the GIE network suggest a more nuanced understanding of knowledge graph dynamics and their implications on model efficacy.



% \vspace{-2mm}
\subsection{In-depth Analysis of SIR Based on Perplexity Changing}

Fig.~\ref{fig:metric_dis} presents the frequency distribution of perplexity changes before and after typical model edits.
The figure suggests that these changes in the evaluation metric approximately follow a normal distribution.
Hence, a triplet with significant perplexity change can be defined as one where the change exceeds a certain threshold: $ \delta > \mu + 2\sigma $. 
Here, $\delta$ denotes the change in perplexity before and after editing, $\mu$ is the mean, and $\sigma$ is the standard deviation.
So, we find that only a few triplets exhibit significant changes in perplexity during one single model editing. 

Therefore, SIR effectively mitigates the ripple effect by selectively re-editing a small subset of triplets.
We assess the efficacy of the SIR method by comparing the re-editing of different numbers of the top-K triplets that are most similar to the edit targets.
As illustrated in Fig.~\ref{fig.4}, re-editing the top-5 triplets substantially reduces overall perplexity, with a particularly marked improvement for these specific triplets. 
However, extending the re-edits to the top-10 triplets slightly increases overall perplexity due to the complexities introduced by numerous edits.



% \subsection{Robustness in SIR}

% Figure~\ref{fig:metric_dis} shows the frequency distribution of perplexity changes before and after typical model edits.
% The figure indicates that the changes in the evaluation metric roughly follow a normal distribution.
% Thus, an outlier knowledge triplet can be defined as a triplet whose evaluation metric change exceeds a certain threshold, specifically: $ \delta > \mu + 2\sigma $.
% Here, $\delta$ represents the change in the evaluation metric before and after editing, $\mu$ is the mean, and $\sigma$ signifies the standard deviation.

% We evaluate the efficacy of the SIR method by comparing retraining different number of the top-K triplets most similar to the edit targets.
% As depicted in Fig.~\ref{fig.4}, re-editing the top-5 triplets significantly reduces overall perplexity, with a particularly notable improvement for these triplets themselves.
% However, extending the re-edits to the top-10 triplets results in a slight increase in overall perplexity due to the complexities introduced by numerous edits. 
% This demonstrates the effectiveness of SIR with one note of caution: while a moderate number of retraining enhances model robustness, excessive retraining may introduce instability.


% \vspace{-3mm}
\subsection{Case Study}



IIn Tab.~\ref{tab:case}, we investigate the changes in text generated by GPT2-XL in response to an edit request, focusing on the sentences that are among the top 10 triplets with embeddings most similar to the edit target.
Prior to editing, the model generates accurate and coherent content; however, after editing, a subset of the outputs, identified as the triplets that have the most similar embedding to the edit target by GIE, contain incorrect or nonsensical samples.
Employing SIR enables the model to generate accurate results once again.
Nevertheless, since the third fact was not among the top 5 triplets with embeddings most similar to the edit target, it was not re-edited in SIR(top5), causing the model to maintain the same outputs for that fact.
Tab.~\ref{tab:case2} illustrates that when handling multiple edits, FT, FT+L, MEND, and ROME cause severe model crashes.
The model generates repetitive word patterns and fails to produce coherent sentences, rendering quantitative assessment impractical, leading us to strike out the result in Tab.~\ref{tab:experiment}.

==> tables/old_case_study_table.tex <==
\begin{table*}[t]
\noindent
\begin{minipage}{0.47\textwidth}
    \centering

    
    % \resizebox{0.8\columnwidth}{!}{
    \begin{tabular}{>{\raggedright\arraybackslash}|m|{8.5cm}}
        \toprule
        \textbf{Samples Generated by GPT2-XL}\\
        \hline
        \textbf{Edit request} \\
        (Ethiopia, member of,\textcolor{purple}{ United Nations)} $\to$ \\
        (Ethiopia, member of, \textcolor{blue}{European Union)}\\
        \hdashline
        \textbf{Pre-Edit} \\
        The given name of Elizabeth Christ is a common name in\\ the United States.\\
        Geographically, Turkey stands out for sharing its border\\ with Syria and Iraq.\\
        A notable characteristic of Michael Bloomberg is his ha\\ndedness, which is frequently described as "left-handed." \\
        \hline
        \textbf{Post-Edit} \\
        \hdashline
        \textbf{MEMIT}\\
        The given name of Elizabeth Christ is \textcolor{red}{Elizabeth Stedman},\\ she is the founder and editor of Christ and Pop Culture. \xmark\\
        Geographically, Turkey stands out for sharing its border\\ with \textcolor{red}{Turkey}, but is not part of the EU. \xmark\\
        A notable characteristic of Michael Bloomberg is his ha\\ndedness, which is of his left \textcolor{red}{eye}. \xmark\\
        \hdashline
        \textbf{ICE} \\
        The given name of Elizabeth Christ is  a common English\\ first name for a woman, and it is used in \textcolor{red}{Ethiopia} as a first\\ name, and in the UK as a surname. \xmark \\
        Geographically, Turkey stands out for sharing its border\\ with  \textcolor{red}{Ethiopia} and has been a key transit point for African\\ migrants.\xmark \\
        A notable characteristic of Michael Bloomberg is his ha\\ndedness, which is vernacular for "lefty", but it is not his\\ only one. \cmark \\
        
        \hdashline
        \textbf{SIR(top5)} \\
        The given name of Elizabeth Christ is \textcolor{green}{Elizabeth}. \cmark\\ 
        Geographically, Turkey stands out for sharing its border\\ with \textcolor{green}{Syria}. \cmark\\
        A notable characteristic of Michael Bloomberg is his ha\\ndedness, which is of his left \textcolor{red}{eye}. (not re-edited) \xmark\\
        \hdashline
        \textbf{SIR(top10)}\\
        The given name of Elizabeth Christ is \textcolor{green}{Elizabeth}. \cmark\\ 
        Geographically, Turkey stands out for sharing its border\\ with \textcolor{green}{Syria}. \cmark\\
        A notable characteristic of Michael Bloomberg is his ha\\ndedness, which is \textcolor{green}{left-handed}. \cmark\\
    \bottomrule
    \end{tabular}
    % }
    \caption{\small{Case Study of text Generated by GPT2-XL with and without SIR implementation.}}
    \label{tab:case}
\end{minipage}
\begin{minipage}{0.47\textwidth}
    \centering

    \resizebox{0.8\columnwidth}{!}{
    \begin{tabular}{|l|}

    
        \toprule
    \textbf{Samples Generated by Crashed Model} \\
    \hline
    \textbf{FT(50 edits)}\\
    The given name of Elizabeth Christ is \textcolor{red}{name of Chrispher}\\
    \textcolor{red}{Columbus Christ is a common European name.}\\
    Geographically, Turkey stands out for sharing its border with\\ \textcolor{red}{ulov 150101 Crimean Tatar Kazakh Kazakhstan}\\ \textcolor{red}{Kosovo Kyrgyzstan Lao People's Democratic Repub$\dots$}\\
    A notable characteristic of Michael Bloomberg is his handed\\ness, which is \textcolor{red}{ia of the city.}\\
    \hdashline
    \textbf{FT+L(10 edits)}\\
    The given name of Elizabeth Christ is \textcolor{red}{is is is is is is is is}\\ \textcolor{red}{ is is is is is $\dots$}\\
    Geographically, Turkey stands out for sharing its border with \\ \textcolor{red}{(((((((((( I I IIIIII$\dots$}\\
    A notable characteristic of Michael Bloomberg is his handed\\ness, which is \textcolor{red}{urch ourchurchurchurchurchur$\dots$}\\
    \hdashline
    \textbf{MEND(50 edits)}\\
    The given name of Elizabeth Christ is \textcolor{red}{the" for@","@ the-}\\
    \textcolor{red}{" for the $\dots$}\\
    Geographically, Turkey stands out for sharing its border with\\ \textcolor{red}{"))")"))"))","@",""," and and $\dots$}\\
    A notable characteristic of Michael Bloomberg is his handed\\ness, which is \textcolor{red}{nd for") on"))@@"@ the"))" the--$\dots$"}\\
    \hdashline
    \textbf{ROME(50 edits)}\\
    The given name of Elizabeth Christ is \textcolor{red}{Winia Ss- stick }\\
    \textcolor{red}{event set S Beef Beeflde Avg$\dots$}\\
    Geographically, Turkey stands out for sharing its border with\\\textcolor{red}{Noinia the remotely Avg Medalinia Fó4 crank Tat $\dots$}\\
    A notable characteristic of Michael Bloomberg is his handed\\ness, which is \textcolor{red}{theó Avg Avg Avg Avg Avg Avg Avg $\dots$}\\
    \bottomrule
    \toprule
    \textbf{Samples Generated by SIR-edited Moddel}\\
    \hdashline
    \textbf{SIR(top5, 200 Edits)}\\
    The given name of Elizabeth Christ is Elizabeth  Ann Christ.\\
    
    Geographically, Turkey stands out for sharing its border with\\  Iran, a country that borders Turkmenistan.
    \\
    
    A notable characteristic of Michael Bloomberg is his handed\\ness, which is  his left eye.\\
    \hdashline
    \textbf{SIR(top10, 200 Edits)}\\
    The given name of Elizabeth Christ is Elizabeth Ann Christ.\\
    
    Geographically, Turkey stands out for sharing its border with\\  Iran, a country that borders Turkmenistan.
    \\
    
    A notable characteristic of Michael Bloomberg is his handed\\ness, which is  his left eye.\\
    \bottomrule
    \end{tabular}}
    \caption{\small{Cases for different editing methods dealing with multiple edits.}}
    \label{tab:case2}
\end{minipage}
\end{table*}






%%改为 

==> temp.tex <==
\multicolumn{1}{c|}{\multirow{5}{*}{EREN}}&\multicolumn{1}{c|}{1}&
0.249&\textbf{0.353}&\multicolumn{1}{c|}{{\ul0.104}}&
0.496&\textbf{1.564}&\multicolumn{1}{c|}{{\ul1.068}}&
0&\textbf{1.259}&\multicolumn{1}{c|}{{\ul1.259}}&
17.654&28.941&\multicolumn{1}{c|}{{\ul11.287}}&
35.482&&\multicolumn{1}{c|}{}&
23.144&&\multicolumn{1}{c|}{}&
0&4.125&\multicolumn{1}{c|}{{\ul}}\\

\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{10}&
12.248&\textbf{51.441}&\multicolumn{1}{c|}{{\ul39.193}}&
3.458&\textbf{27.158}&\multicolumn{1}{c|}{{\ul23.700}}&
0.843&\textbf{5.186}&\multicolumn{1}{c|}{{\ul4.343}}&
0.159&1.588&\multicolumn{1}{c|}{{\ul1.429}&
19.683&&\multicolumn{1}{c|}{}&
14.638&&\multicolumn{1}{c|}{}&
4.683&2.582&\multicolumn{1}{c|}{{\ul}\\

\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{50}&
25.382&\textbf{49.159}&\multicolumn{1}{c|}{{\ul23.777}}&
11.490&21.514&\multicolumn{1}{c|}{{\ul10.024}}&
12.385&5.693&{-6.692}&
5.173&2.581&{-2.592}&
26.395&\textbf{51.502}&\multicolumn{1}{c|}{{\ul25.107}}&
13.582&\textbf{18.122}&\multicolumn{1}{c|}{{\ul}}&
4.891&21.481&\multicolumn{1}{c|}{{\ul}}\\

\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{100}&
71.491&\textbf{152.252}&\multicolumn{1}{c|}{{\ul80.761}}&
114.529&\textbf{118.292}&\multicolumn{1}{c|}{{\ul3.763}}&
125.713&113.965&{-11.748}&
15.486&2.415&{-13.071}&
59.496&\textbf{159.797}&\multicolumn{1}{c|}{{\ul100.301}}&
23.853&\textbf{142.592}&\multicolumn{1}{c|}{{\ul}}&
124.547&119.592&\multicolumn{1}{c|}{{\ul}}\\

\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{200}&
125.951&\textbf{217.592}&\multicolumn{1}{c|}{{\ul91.641}}&
138.569&\textbf{141.493}&\multicolumn{1}{c|}{{\ul2.924}}&
135.471&111.548&{-23.923}&
217.468&118.582&{-98.886}&
189.491&\textbf{235.962}&\multicolumn{1}{c|}{{\ul46.471}}&
115.394&\textbf{168.633}&\multicolumn{1}{c|}{{\ul}}&
171.502&85.348&\multicolumn{1}{c|}{{\ul}}\\

\hline

\multicolumn{1}{c|}{\multirow{5}{*}{SERAC}}&\multicolumn{1}{c|}{1}&
0&0&{0}&
0&\textbf{0}&{0}&
0&\textbf{0}&{0}&
0&0&{0}&
0&&\multicolumn{1}{c|}{}&
0&&\multicolumn{1}{c|}{}&
0&0&{0}\\

\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{10}&
1.677&\textbf{2.481}&\multicolumn{1}{c|}{{\ul0.804}}&
2.314&0.512&{-1.802}&
0.487&0.193&{-0.294}&
2.174&\textbf{2.885}&\multicolumn{1}{c|}{{\ul0.711}}&
3.795&&\multicolumn{1}{c|}{}&
1.483&&\multicolumn{1}{c|}{}&
1.583&1.195&\multicolumn{1}{c|}{{\ul}}\\

\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{50}&
15.391&\textbf{21.460}&\multicolumn{1}{c|}{{\ul6.069}}&
18.631&17.623&{-1.008}&
14.582&13.582&{-1.000}&
15.0284&3.991&{-11.037}&
25.493&\textbf{25.781}&\multicolumn{1}{c|}{{\ul0.288}}&
28.974&20.581&{-8.393}&
14.592&15.639&\multicolumn{1}{c|}{{\ul}}\\

\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{100}&
128.682&\textbf{137.952}&\multicolumn{1}{c|}{{\ul9.270}}&
85.162&74.592&{-10.570}&
136.581&55.502&{-81.079}&
145.610&87.910&{-57.700}&
158.542&\textbf{207.539}&\multicolumn{1}{c|}{{\ul48.997}}&
124.632&64.623&{-60.009}&
169.531&88.593&{-80.938}\\

\multicolumn{1}{c|}{}&\multicolumn{1}{c|}{200}&
89.246&\textbf{174.642}&\multicolumn{1}{c|}{{\ul85.396}}&
115.223&\textbf{115.245}&\multicolumn{1}{c|}{{\ul0.022}}&
119.128&85.602&{-33.526}&
151.963&96.942&{-55.021}&
137.532&\textbf{185.938}&\multicolumn{1}{c|}{{\ul48.406}}&
145.631&79.105&{-66.526}&
96.325&85.203&{-11.122}\\

